Algebraic Smooth Occluding Contours

Computing occluding contours is a key building block of non-photorealistic rendering, but producing contours with consistent visibility has been notoriously challenging. This paper describes the first general-purpose smooth surface construction for which the occluding contours can be computed in closed form. For a given input mesh and camera viewpoint, we produce a $G^1$ piecewise-quadratic surface approximating the mesh. We show how the image-space occluding contours of this representation may then be described as piecewise rational curves. We show that this method produces smooth contours with consistent visibility much more efficiently than the state-of-the-art.

==> figure_tex/overview.tex <==
\begin{figure}
    \centering
%    \picbox{\columnwidth}{1in}
    \caption{\aaron{Overview figure(s) with diagrams illustrating process and representations.  Possibly: Mesh -> Mesh with parametrization -> Projective transform-> Quadratic patches -> Curves in patches -> drawing. RC: Use cat head with two cones; get cone vertices from mesh lab and add directly. Use a small mesh but need at least one or two cones.  }
    \denis{isn't it replicating the teaser to some extent? cut?}
    }
    \label{fig:my_label}
\end{figure}

==> figure_tex/projective.tex <==
\begin{figure}
\centering
\includegraphics[width=0.7\columnwidth]{images/fig-perspective.pdf}
%\picbox{\columnwidth}{1.5in}
%\denis{is fish visible from the ring side?  hard to tell what is going on with it, the teaser is much more obvious}
\caption{3D perspective transformation converting perspective projection frustum to a cube. 
%\aaron{
%* Mesh->Projective transformation visualization (for whichever mesh used in the teaser)
%  perhaps show  projective transform for a couple of camera FOV angles, 
%and for each show both the mesh and the resulting surface. goal: show that we get %reasonable behavior in new surface.  
%- RC: Make 3 for FOV 
%- RC: Create smooth surface -> render from same camera (perspective camera)
%- RC: Apply perspective transformation of mesh -> create smooth surface -> render %(orthographic)
%}
}
\label{fig:projective}
\end{figure}

==> figure_tex/table_stats.tex <==
\begin{table*}[t]
\centering
    \begin{tabular}{|lcc|ccc|ccc|}
      \hline
      &&&\multicolumn{3}{c|}{\bf B\'{e}nard et al.~\shortcite{Benard:2014}} &
      \multicolumn{3}{c|}{\bf Our method} \\ \hline
      \multirow{2}{*}{Sequence} & Input & \multirow{2}{*}{Frames} &
      Output & Inconsistent & Time &
      Output & Inconsistent & Time 
      \\
      &faces&&faces&faces&(sec.)&faces&faces&(sec.)\\
      \hline
      Stanford Bunny & 42,928 & 400 &
      \quad $51,336 \pm 1,383$ & $7.6 \pm 4.4$ & $120 \pm35$ &
      $23,424 \pm518.1$ & 0 & $12 \pm2.2$\\
      Angela's face & 39,576 & 150 &
      \, $50,907 \pm693$ & $14 \pm4.4$& $170 \pm42$ &
      $26,642 \pm6,286$ & 0 & $28 \pm22$ \\
      Walking Man & 30,912 & 120 &
      $158,184 \pm663$ & $2.3 \pm2.1$ & $160 \pm15$ &
      $10,825 \pm2,620$ & 0  & $12 \pm10$\\
%      Yeah Right & 754,688 & 
%      \, $990,589 \pm3654$ & $86 \pm28$ & $1752 \pm489$ &
%      $ \pm$ &   & $ \pm $\\
      \hline
    \end{tabular}
\caption{
\aaron{placeholder: table/caption directly copied from ConTesse}
Statistics of our mesh generation algorithm on three of the animation sequences tested by \cite{Benard:2014}. The ``Red'' animation is omitted because it is proprietary.
The numbers are averaged over animation frames, which we list together with the standard deviation in each case. 
Our method produces no inconsistencies, far fewer output faces (roughly half), and runs much faster ($6\times$ to $13\times$ speedup). These values are for generating front and back faces, though back-faces would almost never be generated in practice.  Details: Both methods were run with a single thread on the same MacBook Pro (3.1GHz Intel Core i5 CPU, 8GB of memory).  The number of input faces is after one round of subdivision, and computation times are for mesh generation only, not stylization. We report fewer input faces for ``Walking Man'' because our method using 1 subdivision level as the minimum subdivision level, rather than 2 subdivisions used by B\'enard et al.}
\label{table:benard}
\end{table*}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "contours"
%%% End: 
